Wav2Pix: Speech-conditioned Face Generation using Generative Adversarial Networks

Speech is a rich biometric signal that contains information about the identity, gender and emotional state of the speaker. In this work, we explore its potential to generate face images of a speaker by conditioning a Generative Adversarial Network (GAN) with raw speech input. We propose a deep neural network that is trained from scratch in an end-to-end fashion, generating a face directly from the raw speech waveform without any additional identity information (e.g reference image or one-hot encoding). Our model is trained in a self-supervised approach by exploiting the audio and visual signals naturally aligned in videos. With the purpose of training from video data, we present a novel dataset collected for this work, with high-quality videos of youtubers with notable expressiveness in both the speech and visual signals.

==> Introduction_old.tex <==
`\section{Introduction}
\amanda{Needs to be shorter}
% -------------------------------------------------
% MOdel Diagram 
%---------------------------------------------------
\begin{figure*}[!ht]
\centering
\includegraphics[width=\textwidth]{ICASSP/architecture.pdf}
\caption{The overall diagram of our speech-conditioned face generation GAN architecture. The network contains an speech encoder, a generator and a discriminator network, respectively represented. Audio embedding (green) is used by both generator and discriminator, but its error is just back-propagated to the generator. It is encoded and projected to a lower dimension (vector of size 128). The pink blocks represent convolutional/deconvolutional stages.}

\label{fig:architecture}
\end{figure*}
%-----------------------------------------------------------------

% ----------------------------------------------------------------
% General info and motivation 
Audio and visual information are the most common modalities used by humans to identify other humans and sense their identity and emotional state.
Features extracted from these two signals are often highly correlated, providing us the capability of imagining the visual appearance of a person just by listening to their voice or building some expectations about the tone or pitch of their voice from just looking to a picture.

% % Challenges
However, when it comes to machines, this multimodal perception is still a direction to be explored. 
Unlike most works on cross-modal analysis that learn a common latent space, image synthesis from multimodal inputs poses further challenges. Apart from creating joint representations exploiting intra-modal correlations, in the case of cross-modality generation it needs to further model details of the samples and learn a complex generative function that produces meaningful outputs. Going one step further than retrieval or zero-shot learning, for generation one has the added challenge of further synthesizing the novel images and/or sounds that have never been seen or heard before.
%Present our idea
In this paper, we focus on the challenge of cross-modal visual generation. More specifically, in the generation of faces conditioned to a given speech signal. 

% Difference from popular works
One of the first approaches to address this task was proposed by Chung \textit{et. al.}, who presented a method for generating a video of a talking face~\cite{said_that}. Their method take as input the Mel-frequency cepstral coefficients (MFCC) of a speech frame of the target speaker (audio) and an image of him/her (identity), and output an image synchronized with the speech. 
Similarly to them, Suwajanakorn \textit{et. al.} synthesized high quality video of President Barack Obama~\cite{obama}. However, they did not generate faces, but images of lips instead. 
Unlike those works, in the proposed approach we aim to a) generate the whole face in an end-to-end fashion, starting from the raw speech signal(without any feature extraction) and b) without providing any identity information (e.g gender or emotion).

% Dataset - needs to be shorter
\amanda{Are we gonna make it available?}
The most common audio-visual datasets used for such tasks are usually build from videos in the cloud. Some of them such as such as \textit{Lip Reading in the wild}~\cite{lrw}, \textit{VoxCeleb}~\cite{voxceleb}, or \textit{VoxCeleb2}~\cite{chung2018voxceleb2} would be suitable for our problem.
However, due to the nature of the video collection process, normally the position of the speaker, the background, and the quality of the videos and the acoustic can significantly vary across different samples in the dataset.
For the particular task of face generation given speech, high quality aligned samples (i.e. the speech should match the person appearing in the video) are needed. To this end, we collected a video dataset from \textit{YouTube}, which is composed of videos uploaded to the platform by well-established users (commonly known as youtubers), who tend to record themselves speaking in front of the camera in their personal home studios. Restricting the dataset to this specific domain we can guarantee high quality recordings, as well as high speech and face expressiveness.

% Contribution
Thus, our main contribution can be summarized as follow:
1) \amanda{We developed a generate adversarial network to generate the whole face in an end-to-end fashion, starting from the raw speech signal(without any feature extraction) and without providing any identity information (e.g gender or emotion) as shown in Figure \ref{fig:architecture}.}
In addition to our dataset, we apply our model to a more challenging faces orientation and speech recording dataset, VoxCeleb~\cite{voxceleb}. 
2) \amanda{We present a novel dataset bla bla bla}







%Although recent generative models achieved to successfully animate faces given an audio input, to the best of our knowledge, this is the first work that is able to generate faces using Generative Adversarial Networks conditioned on the speech signal. \amanda{Double check if it is true!!!!! Maybe some citations about the models?}

%\amanda{To the best of our knowledge this is the first work that achieves to generate images of faces conditioned on speech signal using Generative Adversarial Networks.}



%Deep generative models require large amounts of data to be trained on. Existing publicly available video datasets\cite{voxceleb,youtube8m} have been built by searching for textual queries in video repositories (e.g. \textit{YouTube}) and downloading the matching videos. However, due to the nature of the video collection process, the quality of the videos can significantly vary across different samples in the dataset. Although other datasets have been collected in more restrictive environments \cite{lrw,lrs} these tend to be smaller-scale datasets and have low speaker variability.

%For the particular task of face generation given speech, high quality aligned samples (i.e. the speech should match the person appearing in the video) are needed. To this end, we collected a video dataset from \textit{YouTube}, which is composed of videos uploaded to the platform by well-established users (commonly known as \textit{youtubers}), who tend to record themselves speaking in front of the camera in their personal home studios. Restricting the dataset to this specific domain (i.e. individuals  guarantees high quality recordings, as well as high speech expressiveness. We make this dataset available for download under a novel format: a virtual machine that will download all data from the cloud and run all necessary pre-processing. We believe this approach facilitates the access to the data that facilitates reproducibility and dataset extension in the future.

%------------------------------------------------------------------

%The remainder of the paper is structured as follows. Section \ref{sec:related_work} reviews generative models and other previous works related to image generation. Section \ref{sec:dataset} presents the new dataset and the methodology applied to build it. Section \ref{sec:method} describes the different generative approaches we have explored. Section \ref{sec:exps} includes the qualitative and quantitative results of our experiments. Section \ref{sec:conclusions} concludes with the final outcomes and future research directions.





==> Related_works_old.tex <==
\section{Background}
\amanda{Should we separate Related works from Background? Should the section be called related works and have a subsection called background?}
\amanda{Needs to be reduced!!!!}

% ----------------------------------------------------------
% General explanation about GAN, Contitioned GANs and LSGAN
%-----------------------------------------------------------
Generative Adversarial Networks (GANs) \cite{gan} are a type of generative models that consist in two networks, a Generator $G$ and a Discriminator $D$ that play a min-max game against each other. In this framework, the Generator learns to map samples $z$ coming from some prior distribution $Z$ to samples $x$ from another data distribution characteristics $X$, which comes from the training data (e.g images, audio, etc.). This learning process is possible by means of an adversarial training, where we have another component, the Discriminator. The discriminator is typically a binary classifier which its input are either \textit{real} samples, coming from the dataset, or  \textit{fake} samples generated by $G$.

Another version of this methodology is called Conditional GANs \cite{cGAN} where we give a extra conditional variable $y$ to $G$ and $D$ to perform the mapping  and classification tasks, respectively. 
One particular example can be seem in \cite{textoimage}, where they use conditional GANs to generate images conditioned on text captions.

Although recent improvements in the GANs methodology are presented to stabilize the training process and enhance the quality of the generated samples by $G$, the classic approach commonly suffers from vanishing gradients due to the sigmoid cross-entropy loss used for training.
In order to fix this issue, some approaches \cite{wGan, began, LSGAN} propose changes in the loss function during training.
In the case of the least-squares GAN (LSGAN) approach \cite{LSGAN} proposed to substitute the cross-entropy loss by the least-squares function with binary coding (1 for real, 0 for fake). 
In this case, if we also take into account the additional conditional variable $y$ proposed by \cite{cGAN} the objective function of $D$ and $G$ can be expressed respectively as:

\begin{equation}
\begin{aligned}
  \underset{D}\min~V_{\text{LSGAN}}(D) & = \frac{1}{2}\E_{\ve{x},\ve{y}\sim p_{\text{data}}(\ve{x}, \ve{y})}[(D(\ve{x},\ve{y}) - 1)^{2}]\\
    &+ \frac{1}{2}\E_{\ve{z}\sim p_{\ve{z}}(\ve{z}),\ve{y}\sim p_{\text{data}}(\ve{y})}[D(G(\ve{z},\ve{y}),\ve{y})^{2}].
  \label{eq:lsgan_d}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\underset{G}\min~V_{\text{LSGAN}}(G) = \frac{1}{2}\E_{\ve{z}\sim p_{\ve{z}}(\ve{z}),\ve{y}\sim p_{\text{data}}(\ve{y})}[(D(G(\ve{z},\ve{y}),\ve{y}) - 1)^{2}].
  
\label{eq:lsgan_g}
\end{aligned}
\end{equation}

In this paper, we use a conditional LSGAN to generate faces conditioned to a speech signal.

% -------------------------------------------------
% Related Works
%------------------------------------------------------

\amanda{FIX ME: applications of GANs not using conditional thing
reorder the citations}
\subsection{Related works}

Image synthesis is the most typical and yet interesting application of GANs. 
Followed by that, the combination of multimodal information specially natural language and vision with generative models have driven a lot of attention to the community \cite{DCGAN, textoimage, ACGAN, stackgan}.   

When it comes to the combination of text vision together with generative models, the obvious task that comes into our minds is to generate realistic images from a caption of them. In this direction, \cite{textoimage, stackgan} proposed different approaches to synthesize realistic images given a text description or caption, respectively.

Another path of the cross-modal generation is followed by the computer vision and speech communities to either generate speech from a video \cite{speech_recons} or to generate images from audio/speech \cite{s2i}, in which we will focus. 
However, most work in this field have approached the task with a non-end to end approach, by exploiting a previous knowledge about the data. Typically, speech has been encoded with handcrafted features, such us the MEL spectrum or Mel-frequency Cepstral Coefficients (MFCC), which have been very well engineered to represent human speech. At the visual part, point-based models of the face \cite{karras2017audio} or the lips \cite{obama} have been used to obtain very realistic results. In contrast to that, \textit{Speech2YouTuber} is trained entirely end-to-end from raw speech to pixel images, and no hand-crafted features or additional pre-training is used. 

A direct synthesis of facial pixels was obtained in \cite{said_that} with a discriminative model whose input were a pair of audio feature and a visual example of the face to predict. In this case, the model had the help of this additional identity tower to help in the prediction, so that the deep convolutional network learned how to modify this input to match with the speech utterance. Following a similar architecture, a generative model trained with adversarial training has been recently proposed \cite{e2espeech}, in this case also introducing a temporal regularization to improve the smoothness of the output video sequence. The main difference of \textit{Speech2YouTuber} with these two works is its lack of tower for visual identity, which is learned and encoded in the network parameters during training.

%\cite{s2i} also explored several methods to synthesize images from sound.  To build the sound encoder they tested different sound representations, achieving best results using Log-Amplitude of Mel Spectrum (LMS), and fed a CNN with them.  They projected the resulting sound embedding into a lower dimensional space and concatenated it with the random noise. The rest of the network followed the same architecture as in \cite{textoimage}.

In the previous paragraphs there have been shown different examples of generative methods using audio and images. Nevertheless, all of them were in need of an audio feature extraction before feeding the data to the network. This clearly could limit the network's learning, as we are manually extracting information from the audio.

In contrast, \cite{segan} proposed a method for speech enhancement in which they do not work on the spectral domain, but at the waveform level instead. That means, no hand-crafted features were used to train the network. 
In this method, the generator consists on an encoder-decoder architecture, both of them fully convolutional, and is trained end-to-end. Furthermore, it learns from different speakers and noise types using a single parametrization, reason why it is suitable for generalization in those dimensions. 

%\textit{Speech2YouTuber} applies recent techniques proposed for generative adversarial training to the problem of image generation conditioned by raw speech. In this section we review the basics of conditional adversarial training and the previous works in face synthesis from speech.


% -------------------------------------------------
% MOdel Diagram 
%---------------------------------------------------
\begin{figure*}[!ht]
\centering
\includegraphics[width=\textwidth]{ICASSP/architecture.pdf}
\caption{The overall diagram of our speech-conditioned face generation GAN architecture. The network contains an speech encoder, a generator and a discriminator network, respectively represented. Audio embedding (green) is used by both generator and discriminator, but its error is just back-propagated to the generator. It is encoded and projected to a lower dimension (vector of size 128). The pink blocks represent convolutional/deconvolutional stages.}

\label{fig:architecture}
\end{figure*}
%---------------------------------------------------



% -------------------------------------------------
% General info about generative models - To be used in a ext. version
%------------------------------------------------------
%Deep generative models have attracted wide interests in the past few years. As example of that, Generative Adversarial Networks (GANs) \cite{gan}, Variational Auto-Encoders (VAE) \cite{vae} and Autoregressive Generative Models \cite{pixelrnn} have being explored. As a result of that, there are substantial existing methods investigating the better usage of these models for different applications, such as images synthesis \cite{textoimage}, image-to-image translation \cite{img2imgUnpaired, img2img}, speech and audio synthesis \cite{wavenet, waveGAN} among others.  

% ----------------------------------------------------------
% General explanation about GAN, Contitioned GANs and LSGAN
%-----------------------------------------------------------
%Generative Adversarial Networks (GANs) \cite{gan} are a type of generative models that consist in two networks, a Generator $G$ and a Discriminator $D$ that contest against each other. In this framework, the Generator learns to map samples $z$ coming from some prior distribution $Z$ to samples $x$ from another data distribution characteristics $X$, which comes from the training data (e.g images, audio, etc.). This learning process is possible by means
%of an adversarial training, where we have another component, the Discriminator. The discriminator is typically a binary classifier which its input are either \textit{real} samples, coming from the dataset, or  \textit{fake} samples generated by $G$.
%This adversarial learning is formulated as a min-max game which tries to optimize the following objective:

%\begin{equation}
%\begin{split}
%\label{eq:GANs}
%\min_{G} \max_{D}  V(D,G) = \mathbb{E}_{x\sim p_{data}(\textbf{x})}\left [ %\log \mbox{D}(\textbf{x}) \right ] + \\
%\mathbb{E}_{z\sim p_{z}(\textbf{z})}\left [ \log (1 - \mbox{D(G(\textbf{z}))}) \right ].
%\end{split}
%\end{equation}

%Another version of this methodology is called Conditional GANs \cite{cGAN} where we give a extra conditional variable $y$ to $G$ and $D$ to perform the mapping  and classification tasks, respectively. 
%One particular example can be seem in \cite{textoimage}, where they use conditional GANs to generate images conditioned on text captions.

%\begin{equation}
%\begin{split}
%\label{eq:CGAN}
%\min_{G} \max_{D}  V(D,G) = \mathbb{E}_{x\sim p_{data}(\textbf{x})}\left [ \log \mbox{D}(\textbf{x, y}) \right ] + \\
%\mathbb{E}_{z\sim p_{z}(\textbf{z})}\left [ \log (1 - \mbox{D(G(\textbf{z, y}))}) \right ]
%\end{split}
%\end{equation}

% -------------------------------------------------------------------------


